Complementary and Contrastive Learning for Audio-Visual Segmentation

Audio-Visual Segmentation (AVS) aims to generate pixel-wise segmentation maps that correlate with the auditory signals of objects. This field has seen significant progress with numerous CNN and Transformer-based methods enhancing the segmentation accuracy and robustness. Traditional CNN approaches manage audio-visual interactions through basic operations like padding and multiplications but are restricted by CNNs' limited local receptive field. More recently, Transformer-based methods treat auditory cues as queries, utilizing attention mechanisms to enhance audio-visual cooperation within frames. Nevertheless, they typically struggle to extract multimodal coefficients and temporal dynamics adequately. To overcome these limitations, we present the Complementary and Contrastive Transformer (CCFormer), a novel framework adept at processing both local and global information and capturing spatial-temporal context comprehensively. Our CCFormer initiates with the Early Integration Module (EIM) that employs a parallel bilateral architecture, merging multi-scale visual features with audio data to boost cross-modal complementarity. To extract the intra-frame spatial features and facilitate the perception of temporal coherence, we introduce the Multi-query Transformer Module (MTM), which dynamically endows audio queries with learning capabilities and models the frame and video-level relations simultaneously. Furthermore, we propose the Bi-modal Contrastive Learning (BCL) to promote the alignment across both modalities in the unified feature space. Through the effective combination of those designs, our method sets new state-of-the-art benchmarks across the S4, MS3 and AVSS datasets. Our source code and model weights will be made publicly available at https://github.com/SitongGong/CCFormer

==> Table/Ablation_Study1.tex <==
\begin{table*}[htbp]
  % \begin{minipage}{0.35\textwidth}
  %   \centering
  %   \captionsetup{width=.9\textwidth}
  %   \caption{Early integration module analysis. Combination of AVE and VAE modules outperforms the application of using either module in isolation.}
  %   \label{tab:ablation study of early integration module}
  %   \begin{tabular}{cccc}
  %   \toprule
  %        AVE&VAE& \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
  %        \midrule
  %        & &  65.7& 75.8\\
  %        &{$\surd$}&  66.2& 76.1\\
  %        {$\surd$}&&  \underline{66.4}& \underline{76.5}\\
  %        {$\surd$}&{$\surd$}& \textbf{67.7}&\textbf{77.2}\\
  %   \bottomrule
  %   \end{tabular}
  %   % \vspace{-2mm}
  %   % \vspace{-3mm}
  % \end{minipage}
  \begin{minipage}{0.32\textwidth}
    \centering
    % \caption{\textbf{Number of ICI layers}}
    % \vspace{-2mm}
    % \label{tab: ablation study of number of ICI layers}
    \captionsetup{width=.9\textwidth}
    \caption{Number of ICI layers. Implementation of three ICI layers yields the best performance.}
    \label{tab: ablation study of number of ICI layers}
    \begin{tabular}{ccccc}
    \toprule
        %{Number of Layers}&  \multicolumn{2}{c}{MS3}\\
    \multirow{2}{*}{Num. of \ Layers}&\multicolumn{2}{c}{MS3}&\multicolumn{2}{c}{S4}\\
    &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
        \midrule
         1& 68.5&78.4&&\\
         % \midrule
         2&  \underline{70.3}& \underline{79.6}&&\\
         3& \textbf{70.7}& \textbf{80.5}&&\\
         4& 69.6& 79.5\\
    \bottomrule
    \end{tabular}
    % \vspace{-2mm}
    % \vspace{-3mm}
  \end{minipage}%
  \begin{minipage}{0.35\textwidth}
    \centering
    \captionsetup{width=.9\textwidth}
    \caption{Number of ITI layers. Embedding three ITI layers subsequent to each of the three ICI layers results in optimal performance.}
    \label{tab:ablation study of the number of ITI layers}
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}{*}{Num. of \ Layers}&\multicolumn{2}{c}{MS3}&\multicolumn{2}{c}{S4}\\
    &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         1&  67.8& 78.2&&\\
         %\hline
         2&\underline{69.2}&79.7&&\\
         %\hline
         3&\textbf{70.7}&\textbf{80.5}&&\\
         %\hline
         4&66.8&\underline{76.6}&&\\
 %\multicolumn{2}{c}{Ours}& \textbf{66.08}&\textbf{79.87}\\
 \bottomrule
    \end{tabular}
  \end{minipage}
  \begin{minipage}{0.32\textwidth}
      \centering
       \captionsetup{width=.9\textwidth}
    \caption{Ablative Study of Bi-modal Contrastive Learning. Using the enhanced audio features as another modality leads to best performance.}
    \label{tab:ablation study of bcl}
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}{*}{Another modality}& \multicolumn{2}{c}{MS3} & \multicolumn{2}{c}{S4}\\
         &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         original visual features&  \underline{69.5}& 79.4&&\\
         enhanced visual features&  69.2& \underline{79.5}&&\\
         enhanced audio features (ours)& \textbf{70.7}& \textbf{80.5}&&\\
 %\multicolumn{2}{c}{Ours}& \textbf{66.08}&\textbf{79.87}\\
 \bottomrule
    \end{tabular}
  \end{minipage}

\end{table*}

==> Table/Ablation_Study2.tex <==
\begin{table*}[htbp]
  \begin{minipage}{0.32\textwidth}
    \centering
    \captionsetup{width=.8\textwidth}
    \caption{Overall components analysis. The results demonstrate the effectiveness of our proposed modules.}
    \label{tab: ablation study of all the modules}
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}{*}{Components}& \multicolumn{2}{c}{MS3}& \multicolumn{2}{c}{S4}\\
         &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)& \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
        w/o EIM & 67.7& 78.5 & & \\
        w/o ICI Module& 68.1& 77.5 & & \\
        w/o ITI Module & 68.3 & 78.9 & & \\
        w/o BCL & \underline{69.3}&\underline{78.3} & & \\
        CompFormer & \textbf{70.7}&\textbf{80.5} & & \\
    \bottomrule
    \end{tabular}
  \end{minipage}%
  \begin{minipage}{0.35\textwidth}
    \centering
    \captionsetup{width=.8\textwidth}
    \caption{Query generator analysis. Using the attention mechanism for query generation significantly improves the results.}
    \label{tab: ablation study of query generator}
    \begin{tabular}{ccccc}
    \toprule
         \multirow{2}{*}{Query Generator}& \multicolumn{2}{c}{MS3}& \multicolumn{2}{c}{S4}\\
         &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         w/o Query Generator&  68.1& 76.6&&\\
         Repeat Generator& \underline{68.9}&\underline{78.1}&&\\
         Attention Generator& \textbf{70.7}&\textbf{80.5}&&\\
    \bottomrule
    \end{tabular}
    % \vspace{-1mm}
  \end{minipage}
  \begin{minipage}{0.32\textwidth}
    \centering
    \captionsetup{width=.9\textwidth}
    \caption{Early integration module analysis. Combination of AVE and VAE modules outperforms the application of using either module in isolation.}
    \label{tab:ablation study of early integration module}
    \begin{tabular}{cccccc}
    \toprule
    \multirow{2}{*}{AVE}&\multirow{2}{*}{VAE}&\multicolumn{2}{c}{MS3}&\multicolumn{2}{c}{S4}\\
    & & \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         & &  67.7& 78.5 &&\\
         &{$\surd$}&  \underline{69.1}& \underline{79.6} &&\\
         {$\surd$}&&  68.1& 78.3 &&\\
         {$\surd$}&{$\surd$}& \textbf{70.7}&\textbf{80.5}&&\\
    \bottomrule
    \end{tabular}
  \end{minipage}
\end{table*}

==> Table/ablation_study_ms3_s4_1.tex <==
\begin{table*}[htbp]
\begin{minipage}{0.3\textwidth}
\centering
\captionsetup{width=.8\textwidth}
    \caption{Overall components analysis. The results demonstrate the effectiveness of our proposed modules.}
    \label{tab: ablation study of all the modules}
    \scalebox{0.93}{
        \begin{tabular}{ccccc}
        \toprule
        \multirow{2}{*}{Components}& \multicolumn{2}{c}{MS3}& \multicolumn{2}{c}{S4}\\
             &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)& \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
             \midrule
            w/o EIM & 67.7& \underline{78.5} & \underline{83.8} & \underline{92.3}\\
            w/o ICI Module& 68.1& 77.5 & 83.2& 91.9\\
            w/o ITI Module & 67.4 & 77.8 & 83.1 & 91.8\\
            w/o BCL & \underline{69.3}& 78.3 &83.7 & 92.1\\
            CCFormer& \textbf{70.7}&\textbf{80.5} & \textbf{84.9}& \textbf{92.7}\\
        \bottomrule
        \end{tabular}
        }
\end{minipage}
\begin{minipage}{0.4\textwidth}
    \centering
    \captionsetup{width=.8\textwidth}
    \caption{Query generator analysis. Using the attention mechanism for query generation significantly improves the results.}
    \label{tab: ablation study of query generator}
    \scalebox{0.93}{
    \begin{tabular}{ccccc}
    \toprule
         \multirow{2}{*}{Query Generator}& \multicolumn{2}{c}{MS3}& \multicolumn{2}{c}{S4}\\
         &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         w/o Query Generator&  68.1& 76.6& 84.0&\underline{92.4}\\
         Repeat Generator& \underline{68.9}&\underline{78.1}& \underline{84.2}& 92.3\\
         Attention Generator& \textbf{70.7}&\textbf{80.5}&\textbf{84.9}&\textbf{92.7}\\
    \bottomrule
    \end{tabular}
    }
\end{minipage}
\begin{minipage}{0.3\textwidth}
    \centering
    \captionsetup{width=.9\textwidth}
    \caption{Early integration module analysis. The combination of AVE and VAE modules outperforms the application of using either module in isolation.}
    \label{tab:ablation study of early integration module}
    \scalebox{0.93}{
        \begin{tabular}{cccccc}
        \toprule
        \multirow{2}{*}{AVE}&\multirow{2}{*}{VAE}&\multicolumn{2}{c}{MS3}&\multicolumn{2}{c}{S4}\\
        & & \(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
             \midrule
             & &  67.7& 78.5 & 83.8 & 92.3\\
             &{$\surd$}&  \underline{69.1}& \underline{79.6} & \underline{84.5} & \underline{92.4}\\
             {$\surd$}&&  68.1& 78.3 & 84.2 & 92.3\\
             {$\surd$}&{$\surd$}& \textbf{70.7}&\textbf{80.5}& \textbf{84.9}& \textbf{92.7}\\
        \bottomrule
        \end{tabular}
        }
\end{minipage}
\end{table*}

==> Table/ablation_study_ms3_s4_2.tex <==
\begin{table*}[htbp]
  \begin{minipage}{0.32\textwidth}
    \centering
    % \caption{\textbf{Number of ICI layers}}
    % \vspace{-2mm}
    % \label{tab: ablation study of number of ICI layers}
    \captionsetup{width=.9\textwidth}
    \caption{Number of ICI layers. Implementation of three ICI layers yields the best performance.}
    \label{tab: ablation study of number of ICI layers}
    \scalebox{0.92}{
    \begin{tabular}{ccccc}
    \toprule
        %{Number of Layers}&  \multicolumn{2}{c}{MS3}\\
    \multirow{2}{*}{Num. of \ Layers}&\multicolumn{2}{c}{MS3}&\multicolumn{2}{c}{S4}\\
    &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
        \midrule
         1& 68.5&78.4& 83.8& 92.4\\
         % \midrule
         2&  \underline{70.3}& \underline{79.6}& \underline{84.2}& \underline{92.5}\\
         3& \textbf{70.7}& \textbf{80.5}& \textbf{84.9}& \textbf{92.7}\\
         4& 69.6& 79.5 & 83.8& 92.1\\
    \bottomrule
    \end{tabular}
    }
  \end{minipage}
  \begin{minipage}{0.32\textwidth}
    \centering
    \captionsetup{width=.9\textwidth}
    \caption{Number of ITI layers. Embedding three ITI layers subsequent to each of the three ICI layers results in optimal performance.}
    \label{tab:ablation study of the number of ITI layers}
    \scalebox{0.92}{
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}{*}{Num. of \ Layers}&\multicolumn{2}{c}{MS3}&\multicolumn{2}{c}{S4}\\
    &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         1&  67.8& 78.2& 83.7 & 92.1\\
         %\hline
         2&\underline{69.2}&79.7& \underline{84.2}& 92.4\\
         %\hline
         3&\textbf{70.7}&\textbf{80.5}& \textbf{84.9}& \textbf{92.7}\\
         %\hline
         4&68.5&\underline{79.8}& 83.9 & \underline{92.5}\\
 \bottomrule
    \end{tabular}
    }
  \end{minipage}
  \begin{minipage}{0.35\textwidth}
      \centering
       \captionsetup{width=.9\textwidth}
    \caption{Ablative Study of Bi-modal Contrastive Learning. Using the enhanced audio features as another modality leads to best performance.}
    \label{tab:ablation study of bcl}
    \scalebox{0.92}{
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}{*}{Another modality}& \multicolumn{2}{c}{MS3} & \multicolumn{2}{c}{S4}\\
         &\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)&\(M_{\mathcal{J}}\)&\(M_{\mathcal{F}}\)\\
         \midrule
         ori. visual feat.&  \underline{69.5}& 79.4& 83.9 & 92.4\\
         enh. visual feat.&  69.2& \underline{79.5}& \underline{84.3}& \underline{92.6}\\
         enh. audio feat. (ours)& \textbf{70.7}& \textbf{80.5}& \textbf{84.9}& \textbf{92.7}\\
    \bottomrule
    \end{tabular}
    }
  \end{minipage}
\end{table*}
